Parity-based Cumulative Fairness-aware Boosting

Data-driven AI systems can lead to discrimination on the basis of protected attributes like gender or race. One reason for this behavior is the encoded societal biases in the training data (e.g., females are underrepresented), which is aggravated in the presence of unbalanced class distributions (e.g., "granted" is the minority class). State-of-the-art fairness-aware machine learning approaches focus on preserving the \emph{overall} classification accuracy while improving fairness. In the presence of class-imbalance, such methods may further aggravate the problem of discrimination by denying an already underrepresented group (e.g., \textit{females}) the fundamental rights of equal social privileges (e.g., equal credit opportunity). To this end, we propose AdaFair, a fairness-aware boosting ensemble that changes the data distribution at each round, taking into account not only the class errors but also the fairness-related performance of the model defined cumulatively based on the partial ensemble. Except for the in-training boosting of the group discriminated over each round, AdaFair directly tackles imbalance during the post-training phase by optimizing the number of ensemble learners for balanced error performance (BER). AdaFair can facilitate different parity-based fairness notions and mitigate effectively discriminatory outcomes. Our experiments show that our approach can achieve parity in terms of statistical parity, equal opportunity, and disparate mistreatment while maintaining good predictive performance for all classes.

==> margins.tex <==

AdaFair utilizes confidence scores in the instance weight estimation (c.f., Section~\ref{sec:AdaFair_reweighting}) in contrast to vanilla AdaBoost. 
To demonstrate the impact of confidence scores, we compare AdaFair to a variation that does not use confidence scores (Algorithm~\ref{alg:method} line 8, confidence score $\hat{h}$ is removed); we refer to this as AdaFair NoConf, hereafter. We also include vanilla AdaBoost in the comparison. We evaluate the three approaches w.r.t their cumulative margins for each fairness notions. 
\rev{Comparing to accuracy and balanced accuracy that rely only on correctly and incorrectly classifications, the margins also reveal information about how confident are the predictions of the different methods~\cite{schapire2013explaining}. The margin values lie in the $[-1, 1]$ range (x-axis); values close to $-1$ indicate misclassifications with high confidence whereas values close to $1$ indicate correct classifications with high confidence (the y-axis shows the fraction of data). The bulk of the distribution is located where the curve increases abruptly. Similar to the previous experiment, we only show the results on disparate mistreatment and encourage the interested readers to see the Appendix section for the results w.r.t statistical parity and equal opportunity. The cumulative distribution of margins for each dataset and per class is provided in Figure~\ref{fig:cdf_and_weights_eqodds} for disparate mistreatment.}


\begin{figure*}[t!]
  \begin{subfigure}[t]{\textwidth}
  \centering
 \includegraphics[width=.95\columnwidth]{Images/CDF/cdf_adult-gender.png}\vspace{-0.3cm}
 \caption{Adult census} 
 \end{subfigure}
  \begin{subfigure}[t]{\textwidth}
  \centering
 \includegraphics[width=.95\columnwidth]{Images/CDF/cdf_bank.png}\vspace{-0.3cm}
 \caption{Bank} 
 \end{subfigure}
 \centering
 \begin{subfigure}[t]{\textwidth}
  \centering
 \includegraphics[width=.95\columnwidth]{Images/CDF/cdf_compass-gender.png}\vspace{-0.3cm}
 \caption{Compass}
 \end{subfigure}
  \begin{subfigure}[t]{\textwidth}
  \centering
 \includegraphics[width=.95\columnwidth]{Images/CDF/cdf_kdd.png}\vspace{-0.3cm}
 \caption{KDD census} 
 \end{subfigure}
 \caption{Disparate Mistreatment: cumulative distribution of margins}
 \label{fig:cdf_and_weights_eqodds}
\end{figure*}



\noindent\textbf{Disparate Mistreatment:} 
\rev{Based on the results in Figure~\ref{fig:cdf_and_weights_eqodds}, we observe that for the positive class AdaFair is more confident comparing to the other approaches (its curve is shifted to the right) and this holds for all datasets except for Compass where there is no clear winner between AdaFair and AdaFair NoConf - recall that this dataset is balanced. For Adult census dataset the difference is not big since it does not suffer from extreme class imbalance in contrast to Bank and KDD census dataset.} Also, we can observe that AdaFair has the lowest errors in the positive class and the misclassifications in this class have lower confidence values comparing to the other methods. 
Regarding the negative class, we can observe that AdaBoost achieves the best performance compared to AdaFair and AdaFair NoConf, since it focuses solely on overall accuracy, thus it learns better the majority class. 
The differences in the performances of the different methods increase with the dataset imbalance; for example for the \emph{Bank dataset}, AdaFair has significantly less misclassifications in the positive class comparing to AdaFair NoConf ($15\% \downarrow$) and AdaBoost ($36\% \downarrow$), and only small increase in the misclassifications of the negative class, $5\% \downarrow$ and $7\% \downarrow$, respectively.
Similarly, for the KDD census dataset, AdaFair has $23\% \downarrow$ and $46\% \downarrow$ less misclassifications than AdaFair NoConf and AdaBoost, respectively, while the increase in error at the negative class is $12\% \downarrow$ and $14\% \downarrow$, respectively. 
In this case, AdaBoost classifies correctly almost all the negative (majority) instances, but its performance on the minority class is the worst (it has the leftmost curve).


\noindent\textbf{Conclusion:} To conclude, considering confidence scores for instance weight estimation, the ensemble's margins increase especially in case of class imbalance. 
Instead of ``boosting'' all misclassified instances equally, this approach differentiates based on the confidence score of the misclassification, s.t. misclassified instances close to the decision boundary are weighted less than those that are further away.





